Adversarial Attack on Radar-based Environment Perception Systems

Due to their robustness to degraded capturing conditions, radars are widely used for environment perception, which is a critical task in applications like autonomous vehicles. More specifically, Ultra-Wide Band (UWB) radars are particularly efficient for short range settings as they carry rich information on the environment. Recent UWB-based systems rely on Machine Learning (ML) to exploit the rich signature of these sensors. However, ML classifiers are susceptible to adversarial examples, which are created from raw data to fool the classifier such that it assigns the input to the wrong class. These attacks represent a serious threat to systems integrity, especially for safety-critical applications. In this work, we present a new adversarial attack on UWB radars in which an adversary injects adversarial radio noise in the wireless channel to cause an obstacle recognition failure. First, based on signals collected in real-life environment, we show that conventional attacks fail to generate robust noise under realistic conditions. We propose a-RNA, i.e., Adversarial Radio Noise Attack to overcome these issues. Specifically, a-RNA generates an adversarial noise that is efficient without synchronization between the input signal and the noise. Moreover, a-RNA generated noise is, by-design, robust against pre-processing countermeasures such as filtering-based defenses. Moreover, in addition to the undetectability objective by limiting the noise magnitude budget, a-RNA is also efficient in the presence of sophisticated defenses in the spectral domain by introducing a frequency budget. We believe this work should alert about potentially critical implementations of adversarial attacks on radar systems that should be taken seriously.

==> sections/Proposed.tex <==

In this section, we present the proposed attack under two different settings: The first is a baseline attack that generates adversarial noise to specific signals. We discuss the limits of this attack and present a new robust attack that is efficient regardless of the sample, and whether the noise is synchronized with the raw signal or not.



%---------------------
\subsubsection{Fourier Analysis of the Spectral Signature}
%---------------------

We present the corresponding frequency spectrum obtained using the discrete Fourier transform (DFT), which is defined by
\begin{equation}
    F(k) = \sum^{N-1}_{n=0}f(n)e^{-j\frac{2\pi}{N}nk}
\end{equation}
Where $N$ is the length of the spectral signature and $f$ is the original discret signal.
%share similar frequency spectrum signatures
We notice that the clean signal and the adversarial signal have similar frequency spectrum (see Figure \ref{Fig:freq}) meaning that the two signals contain similar range of frequencies. That could be explained by the fact that the same data distribution is used to generate the adversarial noise and %investigate!

\begin{figure*}[t!]
\centering
\includegraphics[width=2\columnwidth]{figures/frequency_spectrum.png}
\caption{ Frequency spectrum of clean and adversarial signals.  -- \textcolor{red}{-- I'm still wondering why we had a noise in the same spectral range, any impact of the loss function or the distance metric ? we might investigate this if we have time }}
\label{Fig:freq}
\end{figure*}

%---------------------
\subsubsection{Impact of applying Filters}
%---------------------

We use the FGSM to attack the victim model with a noise magnitude equal to $0.002$. We try filtering the adversarial signal using the Bessel and Chebyshev type I filters while varying the normalized cut-off frequency $wn$. 

\begin{itemize}
    \item Bessel filter is optimized to provide a constant group delay in the filter passband, while sacrificing sharpness in the magnitude response. 
    %\item Butterworth filter designed to have a frequency response that is as flat as possible in the passband.
    \item Chebyshev type I filter have a steeper roll-off than Butterworth filters, and have passband ripple.
\end{itemize}

We notice that when filtering we lose important information, which leads to a drop in baseline classification accuracy. For instance, when using the Chebyshev type I filter and with a $wn = 0.7$, we had $54\%$ drop in baseline accuracy while only gaining $5\%$ in terms of robustness.

\begin{table}[h]
\small \centering
  \caption{Accuracy results when using filters on clean and adversarial signals.}
  \label{filters}
  \begin{tabular}{ccccc}
    \toprule
    \textbf{Filters} & \multicolumn{2}{c}{\textbf{Bessel}}  &  \multicolumn{2}{c}{\textbf{Chebyshev type I}}\\
    \midrule
    \textbf{$wn$} & \textbf{Clean} & \textbf{Adversarial}& \textbf{Clean} & \textbf{Adversarial} \\
    \midrule
         0.9  & 99\% &  11\%  &  99\% &  10\%   \\
         0.8  & 74\% &   10\% &  95\% &   9\% \\
         0.7  & 62\% &  32\%  &  45\% &  15\% \\
         0.6  & 61\% &  51\%  &  33\% &  20\%  \\
         0.5  & 44\% &  40\%  &  55\% &  40\%  \\
         %0.4  & 39\% &  39\%  &  17\% &  32\% \\
  \bottomrule
\end{tabular}
\end{table}

%---------------------
\subsubsection{Impact of de-synchronization}
%---------------------
We use the baseline attacks (i.e., FGSM and PGD attacks) and the universal adversarial perturbations (UAP) \cite{Universal} to generate adversarial noise and investigate the impact of synchronization on noise effectiveness/ attack success rate. The attack success rate/ effectiveness is defined as  (1 - Classification Accuracy) and represents the proportion of total perturbed signals for which the adversarial noise forces the model to output a wrong label.
UAP are input-agnostic perturbations, when added to an input (image/signal), causes misclassification of the perturbed input. 

We perform random shifts when diffusing the adversarial noise, we notice a huge drop in attack effectiveness (see Table \ref{synch_rand}). In fact, the baseline attacks (with $epsilon = 0.002$) are totally neutralized and for universally trained noises (with $epsilon = 0.01$), we notice a drop from $78\%$ to $37\%$. These attacks require perfect synchronization in order to be effective which is not practical as usually it's hard for the attacker to predict the exact time the system starts to receive the signal.

\begin{table}[h]
\small \centering
  \caption{Attack effectiveness for synchronized and de-synchronized adversarial noise.}
  \label{synch_rand}
  \begin{tabular}{ccc}
    \toprule
    \textbf{Attack}  & \textbf{Synchronized} &  \textbf{De-synchronized}\\
    \midrule
         FGSM            &  93\% &  2\%   \\
         PGD             &  97\% &  1\%   \\
         FGSM-based UAP  &  77\% &  35\%  \\
         PGD-based UAP  &  78\% &  37\%   \\
  \bottomrule
\end{tabular}
\end{table}

%---------------------
\subsection{Unsynchronized noise}
%---------------------

%\textcolor{red}{ -- The algorithm needs to be presented as kinda adapted to our case, and not just a generic one, random locations, etc-- }
As previously shown, a slight timing shift when broadcast the adversarial noise neutralizes the attack even when using the universally trained ones. In order to overcome this issue, we improve \cite{Universal} to generate patches not only input-agnostic but also time-agnostic that can be applied at anytime and still be effective.
Our main objective is to fool a victim model $C(.)$ on almost all the input signals belonging to $\mu$ a distribution of signals in $\mathbb{R}$ \emph{any time} the adversarial noise is diffused. This problem can be formulated as finding a vector $\delta$ such that:

\begin{equation}
    C(x + mask(\delta, k)) \neq C(x), ~ for ~ almost ~ all ~ x \in \mu
\end{equation}

$\delta$ must satisfy the following constraint: $\left\Vert \delta \right\Vert_p \leq \epsilon $. The parameter $\epsilon$ controls the magnitude of the noise vector $\delta$. 
$mask$ is a function that creates a patch from $\delta$ with a location $k$ with respect to the input signal $x_i$ that will be added later on to $x_i$.
Our proposed Algorithm \ref{patch} iterates across the data in the signal sample set $X$ gradually updating our patch. At each iteration, the minimal perturbation $\Delta \delta_i$ is computed using $attack$ which is either FGSM or PGD attack for a specific randomly chosen location k and then aggregated to the current instance of the patch. 

\begin{algorithm}
\caption{Computation of proposed patch.}
\label{patch}
\begin{algorithmic}[1]
\State \textbf{Input:} Data points $X$, classifier $C$, $l_p$ desired norm, $\epsilon$ noise magnitude, $k$ a random location, $N$ number of iterations.
\State \textbf{Output:} $\delta$ trained patch.

\State Initialize $\delta \leftarrow 0$
\While{$iter < N$ }
    \For{each data point $x_i \in X$}
        \If{$C(x_i + mask(\delta, k)) = C(x_i)$}
            \State Select a random location $k$
            \State $\Delta\delta_i \leftarrow  attack(C, x_i + mask(\delta, k), y_i, \epsilon, l_p)$ %\textcolor{blue}{mask() and attack() are functions that need definition. NB: This is the core novelty of the proposed approach --}
            %\State \textit{// Update the patch:}
            \State $\delta \leftarrow \mathcal{P}_{l_p, \epsilon}(\delta + \Delta \delta_i)$
\EndIf
\EndFor
\EndWhile

\end{algorithmic}
\end{algorithm}
%--------------------------------------------------
\begin{algorithm}
\caption{$mask$ function.}
\label{mask}
\begin{algorithmic}[1]
\State \textbf{Input:} $\delta$ patch, $len$ noise length, $k$ a random location, $maxlen$ input signal length.
\State \textbf{Output:} $Mask$ patch at position $k$.

\State Initialize $Mask \leftarrow 0$
\If{$k <= maxlen - len$}
    \State $Mask = Padding(\delta, (k, maxlen - (k + len)), (0,0))$
\Else
    \State $Mask = Append(zeros(k), \delta [0 : maxlen - k])$
\EndIf
\end{algorithmic}
\end{algorithm}
%-------------------------------------------------
\begin{algorithm}
\caption{$attack$ function.}
\label{proposed_pgd}
\begin{algorithmic}[1]
\State \textbf{Input:} a classifier $C$ with loss $J$, noise budget  $\epsilon$, step size $\alpha$, $x$ input image, $y$ label, $m$ number of iterations, $k$ random position, $len$ noise length, $attack$ attack PGD or FGSM
\State \textbf{Output:} $\delta$
\State Initialize~ $\delta \leftarrow 0$
\State Initialize~ $x_{adv} \leftarrow 0$
\If{attack = "PGD"}
    \For {i= 0...m-1}
        \State prediction = $argmax(C(x_{adv})) $
        \State $x_{adv} = Clip \{x + \alpha sign (\nabla_{x_{adv}}J_{\theta}(C(x_{adv}),y)) \times mask(ones(len),k) \}$
    \EndFor
\Else
        \State prediction = $argmax(C(x_{adv})) $
        \State $x_{adv} = x + \epsilon sign (\nabla_{x_{adv}}J_{\theta}(C(x_{adv}),y)) \times mask(ones(len),k)$
\EndIf
\State $\delta = x_{adv} - x$
\end{algorithmic}
\end{algorithm}

%---------------------          
\subsubsection{Impact of Patch length}  
%---------------------
We run an experiment where we change the patch length and investigate its impact on model accuracy. We use algorithm \ref{patch} to train the patches. 
For each test sample, only one patch is diffused at a random time with different noise magnitude ($epsilon$). We notice that the larger the length of the patch, the more powerful the patch (see Figure \ref{Fig:patchSize}).

\begin{figure*}[t!]
\centering
\includegraphics[width=2\columnwidth]{figures/patch_sizevseffectiveness.png}
\caption{Impact of patch length on patch effectiveness under different noise magnitude constraints. }
\label{Fig:patchSize}
\end{figure*}

%---------------------
\subsubsection{Impact of repeating the patch}
%---------------------
In this experiment, we generate patches with different lengths and under different noise magnitude constraints. The patch is then broadcast continuously. We notice an increase in the success rate of the attack up to $90\%$.
The patch length is no longer relevant, as illustrated in Figure \ref{Fig:contbroad}. For instance, even a patch with a length $1/22$ of the total raw signal length can achieve $90\%$ success.

\begin{figure*}[t!]
\centering
\includegraphics[width=2\columnwidth]{figures/repeat_patch.png}
\caption{Continuously broadcast patch effectiveness under different noise magnitude constraints.}
\label{Fig:contbroad}
\end{figure*}


%---------------------
\subsection{Defense mechanism}
%---------------------

Adversarial training (AT) \cite{madry2019deep} is a popular and effective defense strategy in which adversarial noises are generated through an adversarial attack, the noises are added to the inputs, and the clean images (without adversarial noises) and the noisy images (added with adversarial noises) are used to train a DNN model.
A DNN model can learn features of adversarial samples through adversarial training, and by that the classification decision boundary is adjusted so that adding a small amount of adversarial noise makes it difficult to "push" the input samples (images or signals) across the decision boundary.
We used the PGD algorithm \cite{pgd} to implement the white-box adversarial
attacks, a widely used technique for robustness evaluation \cite{tramer2020adaptive}. We set the noise magnitude (epsilon) equal to $0.002$ with a step size of $0.0005$ with a number of iterations equal to $20$. We train the model for $500$ epochs to reach $99\%$ classification accuracy on clean input samples.

In Figure \ref{Fig:AT}, we report the difference in impact of our proposed patches on adversarially-trained models and undefended models in the case of one random localized patch. AT decreases the effectiveness of our attack method for smaller epsilon, however it is practically ineffective for larger epsilons.

\begin{figure*}[t!]
\centering
\includegraphics[width=2\columnwidth]{figures/defense_AT.png}
\caption{Impact of adversarial training (AT) on patch effectiveness.}
\label{Fig:AT}
\end{figure*}

Same trend was noticed for the case of continuously diffused/broadcast patches AT is only effective for smaller noise magnitudes (see Figure \ref{Fig:ATcontbroad}).
\begin{figure*}[t!]
\centering
\includegraphics[width=2\columnwidth]{figures/defense_AT_continu.png}
\caption{Impact of adversarial training (AT) on continuously broadcast patch effectiveness.}
\label{Fig:ATcontbroad}
\end{figure*}

